On Optimal Partitioning For Sparse Matrices In Variable Block Row Format

The Variable Block Row (VBR) format is an influential blocked sparse matrix format designed for matrices with shared sparsity structure between adjacent rows and columns. VBR groups adjacent rows and columns, storing the resulting blocks that contain nonzeros in a dense format. This reduces the memory footprint and enables optimizations such as register blocking and instruction-level parallelism. Existing approaches use heuristics to determine which rows and columns should be grouped together. We show that finding the optimal grouping of rows and columns for VBR is NP-hard under several reasonable cost models. In light of this finding, we propose a 1-dimensional variant of VBR, called 1D-VBR, which achieves better performance than VBR by only grouping rows. We describe detailed cost models for runtime and memory consumption. Then, we describe a linear time dynamic programming solution for optimally grouping the rows for 1D-VBR format. We extend our algorithm to produce a heuristic VBR partitioner which alternates between optimally partitioning rows and columns, assuming the columns or rows to be fixed, respectively. Our alternating heuristic produces VBR matrices with the smallest memory footprint of any partitioner we tested.

==> VBR arxiv/1dvbr_example.tex <==
\resizebox{0.5\width}{!}{$\left[\begin{array}{ccccccccc}\cline{3-3} \cline{4-4} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{5-5} \cline{6-6} \cline{7-7} \cline{9-9} 
\end{array}\right]$}

\subcaption{The stored entries of $A$ in 1D-VBR format. Here, $\Pi = [1{:}1, 2{:}4, 5{:}6, 7{:}8]$.}\label{fig:1dvbr-example}


==> VBR arxiv/bcsr_example.tex <==
\resizebox{0.5\width}{!}{$\left[\begin{array}{ccccccccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\end{array}\right]$}

\subcaption{The stored entries of $A$ in BCSR format. The block size is $2 \times 3$.}\label{fig:bcsr-example}


==> VBR arxiv/csrsimd_example.tex <==
\resizebox{0.5\width}{!}{$\left[\begin{array}{cccccccccccc}\cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{9-9} \cline{10-10} \cline{11-11} \cline{12-12} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} \cline{10-10} \cline{11-11} \cline{12-12} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} \cline{10-10} \cline{11-11} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\\cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} \cline{9-9} \cline{10-10} \cline{11-11} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} \cline{10-10} \cline{11-11} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} \cline{10-10} \cline{11-11} \cline{12-12} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} \cline{10-10} \cline{11-11} \cline{12-12} 
\end{array}\right]$}

\subcaption{The stored entries of $A$ in CSR-SIMD format.}\label{fig:csrsimd-example}


==> VBR arxiv/cutgadget.tex <==
\[
\begin{array}{cc}\makecell{v_i \in V_1 \\ \Pi=[1{:}2, 3{:}3]} & 
\left[\begin{array}{ccc}\cline{1-1} \cline{2-2} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{3-3} 
\end{array}\right]
\\ & 
\\ \makecell{v_{i'} \in V_2 \\ \Pi=[1{:}1, 2{:}3]} &
\left[\begin{array}{ccc}\cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\end{array}\right]
\\ & 
\\ & e_j, \Phi=[1{:}2, 3{:}3]
\end{array}
\text{ or }
\begin{array}{c} 
\left[\begin{array}{ccc}\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}\\
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\\cline{2-2} \cline{3-3} 
\end{array}\right]
\\
\\
\left[\begin{array}{ccc}\cline{2-2} \cline{3-3} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\end{array}\right]
\\
\\e_j, \Phi=[1{:}1, 2{:}3]
\end{array}
\]


==> VBR arxiv/cutgadget2.tex <==
\[
\begin{array}{cc}\makecell{v_i \in V_1, \Pi \\ = [1{:}3, 4{:}4]} & 
\left[\begin{array}{cccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{0}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\end{array}\right]
\\ & 
\\ \makecell{v_{i'} \in V_2, \Pi \\ = [1{:}1, 2{:}4]} &
\left[\begin{array}{cccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\end{array}\right]
\\ & 
\\ & e_j, \Phi = [1{:}3, 4{:}4]
\end{array}
\text{ or }
\begin{array}{c} 
\left[\begin{array}{cccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\\cline{2-2} \cline{3-3} \cline{4-4} 
\end{array}\right]
\\
\\
\left[\begin{array}{cccc}\cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\end{array}\right]
\\
\\e_j, \Phi = [1{:}1, 2{:}4]
\end{array}
\]


==> VBR arxiv/gadget.tex <==
\subsection{Exhaustively Checking \eqref{eq:happygadget}}\label{app:vbrblockingnphard:happygadget}
\paragraph{$\Pi = [1{:}1, 2{:}3, ...], \Phi = [1{:}1, 2{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (5 + 6\mu_2 + 6\mu_3) + (2 + 4\mu_2 + 4\mu_3)s\\
&= 197 + 6\lceil 28s - 10\rceil + (130 + 4\lceil 28s - 10\rceil)s\\
&\leq 143 + 262s + 112s^2
\\&\leq 146 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}1, 2{:}3, ...], \Phi = [1{:}2, 3{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (8 + 6\mu_2 + 6\mu_3) + (3 + 4\mu_2 + 4\mu_3)s\\
&= 200 + 6\lceil 28s - 10\rceil + (131 + 4\lceil 28s - 10\rceil)s\\
&\leq 146 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}2, 3{:}3, ...], \Phi = [1{:}1, 2{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (8 + 6\mu_2 + 6\mu_3) + (3 + 4\mu_2 + 4\mu_3)s\\
&= 200 + 6\lceil 28s - 10\rceil + (131 + 4\lceil 28s - 10\rceil)s\\
&\leq 146 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}2, 3{:}3, ...], \Phi = [1{:}2, 3{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (5 + 6\mu_2 + 6\mu_3) + (2 + 4\mu_2 + 4\mu_3)s\\
&= 197 + 6\lceil 28s - 10\rceil + (130 + 4\lceil 28s - 10\rceil)s\\
&\leq 143 + 262s + 112s^2
\\&\leq 146 + 263s + 112s^2
\end{align*}
\subsection{Exhaustively Checking \eqref{eq:sadgadget}}\label{app:vbrblockingnphard:sadgadget}
\paragraph{$\Pi = [1{:}3, ...], \Phi = [1{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (9 + 6\mu_2 + 12\mu_3) + (1 + 2\mu_2 + 4\mu_3)s\\
&= 201 + 12\lceil 28s - 10\rceil + (65 + 4\lceil 28s - 10\rceil)s\\
&\geq 81 + 361s + 112s^2
\\&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}3, ...], \Phi = [1{:}1, 2{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (9 + 6\mu_2 + 9\mu_3) + (2 + 3\mu_2 + 4\mu_3)s\\
&= 201 + 9\lceil 28s - 10\rceil + (98 + 4\lceil 28s - 10\rceil)s\\
&\geq 111 + 310s + 112s^2
\\&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}3, ...], \Phi = [1{:}2, 3{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (9 + 6\mu_2 + 9\mu_3) + (2 + 3\mu_2 + 4\mu_3)s\\
&= 201 + 9\lceil 28s - 10\rceil + (98 + 4\lceil 28s - 10\rceil)s\\
&\geq 111 + 310s + 112s^2
\\&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}3, ...], \Phi = [1{:}1, 2{:}2, 3{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (9 + 6\mu_2 + 8\mu_3) + (3 + 4\mu_2 + 4\mu_3)s\\
&= 201 + 8\lceil 28s - 10\rceil + (131 + 4\lceil 28s - 10\rceil)s\\
&\geq 121 + 315s + 112s^2
\\&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}1, 2{:}3, ...], \Phi = [1{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (9 + 6\mu_2 + 9\mu_3) + (2 + 3\mu_2 + 4\mu_3)s\\
&= 201 + 9\lceil 28s - 10\rceil + (98 + 4\lceil 28s - 10\rceil)s\\
&\geq 111 + 310s + 112s^2
\\&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}1, 2{:}3, ...], \Phi = [1{:}1, 2{:}2, 3{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (5 + 6\mu_2 + 5\mu_3) + (3 + 5\mu_2 + 4\mu_3)s\\
&= 197 + 5\lceil 28s - 10\rceil + (163 + 4\lceil 28s - 10\rceil)s\\
&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}2, 3{:}3, ...], \Phi = [1{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (9 + 6\mu_2 + 9\mu_3) + (2 + 3\mu_2 + 4\mu_3)s\\
&= 201 + 9\lceil 28s - 10\rceil + (98 + 4\lceil 28s - 10\rceil)s\\
&\geq 111 + 310s + 112s^2
\\&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}2, 3{:}3, ...], \Phi = [1{:}1, 2{:}2, 3{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} \cline{9-9} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (5 + 6\mu_2 + 5\mu_3) + (3 + 5\mu_2 + 4\mu_3)s\\
&= 197 + 5\lceil 28s - 10\rceil + (163 + 4\lceil 28s - 10\rceil)s\\
&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}1, 2{:}2, 3{:}3, ...], \Phi = [1{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (9 + 6\mu_2 + 8\mu_3) + (3 + 4\mu_2 + 4\mu_3)s\\
&= 201 + 8\lceil 28s - 10\rceil + (131 + 4\lceil 28s - 10\rceil)s\\
&\geq 121 + 315s + 112s^2
\\&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}1, 2{:}2, 3{:}3, ...], \Phi = [1{:}1, 2{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{7-7} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (5 + 6\mu_2 + 5\mu_3) + (3 + 5\mu_2 + 4\mu_3)s\\
&= 197 + 5\lceil 28s - 10\rceil + (163 + 4\lceil 28s - 10\rceil)s\\
&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}1, 2{:}2, 3{:}3, ...], \Phi = [1{:}2, 3{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{2-2} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (5 + 6\mu_2 + 5\mu_3) + (3 + 5\mu_2 + 4\mu_3)s\\
&= 197 + 5\lceil 28s - 10\rceil + (163 + 4\lceil 28s - 10\rceil)s\\
&\geq 147 + 263s + 112s^2
\end{align*}
\paragraph{$\Pi = [1{:}1, 2{:}2, 3{:}3, ...], \Phi = [1{:}1, 2{:}2, 3{:}3, ...]$}
\[
\left[\begin{array}{cccccccccc}\cline{1-1} \cline{5-5} \cline{7-7} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{1-1} \cline{2-2} \cline{5-5} \cline{7-7} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{\cdots}\\\cline{2-2} \cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{\cdots}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{\cdots}\\\cline{3-3} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} 
\multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{\vdots}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
\]
\begin{align*}
f(B_1, \Pi, \Phi) &= N_{\text{value}} + N_{\text{index}}s\\
&= (9 + 6\mu_2 + 4\mu_3) + (3 + 6\mu_2 + 4\mu_3)s\\
&= 201 + 4\lceil 28s - 10\rceil + (195 + 4\lceil 28s - 10\rceil)s\\
&\geq 161 + 267s + 112s^2
\\&\geq 147 + 263s + 112s^2
\end{align*}


==> VBR arxiv/notcutgadget.tex <==
\[
\begin{array}{cc}\makecell{v_i \in V_1 \\ \Pi=[1{:}2, 3{:}3]} & 
\left[\begin{array}{ccc}\cline{1-1} \cline{2-2} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{3-3} 
\end{array}\right]
\\ & 
\\ \makecell{v_{i'} \in V_1 \\ \Pi=[1{:}2, 3{:}3]} &
\left[\begin{array}{ccc}\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} 
\end{array}\right]
\\ & 
\\ & e_j, \Phi=[1{:}2, 3{:}3]
\end{array}
\text{ or }
\begin{array}{c} 
\left[\begin{array}{ccc}\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}\\
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\\cline{2-2} \cline{3-3} 
\end{array}\right]
\\
\\
\left[\begin{array}{ccc}\cline{2-2} \cline{3-3} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} 
\end{array}\right]
\\
\\e_j, \Phi=[1{:}1, 2{:}3]
\end{array}
\]


==> VBR arxiv/notcutgadget2.tex <==
\[
\begin{array}{cc}\makecell{v_i \in V_1, \Pi \\ = [1{:}3, 4{:}4]} & 
\left[\begin{array}{cccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{0}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\end{array}\right]
\\ & 
\\ \makecell{v_{i'} \in V_1, \Pi \\ = [1{:}3, 4{:}4]}&
\left[\begin{array}{cccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\end{array}\right]
\\ & 
\\ & e_j, \Phi = [1{:}3, 4{:}4]
\end{array}
\text{ or }
\begin{array}{c} 
\left[\begin{array}{cccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\\cline{2-2} \cline{3-3} \cline{4-4} 
\end{array}\right]
\\
\\
\left[\begin{array}{cccc}\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} 
\end{array}\right]
\\
\\e_j, \Phi = [1{:}1, 2{:}4]
\end{array}
\]


==> VBR arxiv/results/matrices.tex <==
\setlength{\tabcolsep}{2pt}\begin{tabular}{c@{\hspace{1pt}}ccc}
Spy & \makecell{Zoomed \\ Spy} & \makecell{Group / Name \\ $m \times n$ ($N$)} \\ \hline \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/GHS_indef/exdata_1/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/GHS_indef/exdata_1/micro_spy_1477_1477.png}} & \makecell{ GHS\_indef/ \\ \quad exdata\_1 \\ $6001 \times 6001$ ($2269501$)} \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Goodwin/Goodwin_071/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Goodwin/Goodwin_071/micro_spy_910_910.png}} & \makecell{ Goodwin/ \\ \quad Goodwin\_071 \\ $56021 \times 56021$ ($1797934$)} \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Hamm/scircuit/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Hamm/scircuit/micro_spy_55649_55649.png}} & \makecell{ Hamm/ \\ \quad scircuit \\ $170998 \times 170998$ ($958936$)} \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Janna/Emilia_923/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Janna/Emilia_923/micro_spy_8116_8116.png}} & \makecell{ Janna/ \\ \quad Emilia\_923 \\ $923136 \times 923136$ ($41005206$)} \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Janna/Geo_1438/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Janna/Geo_1438/micro_spy_565671_565671.png}} & \makecell{ Janna/ \\ \quad Geo\_1438 \\ $1437960 \times 1437960$ ($63156690$)} \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/LPnetlib/lpi_gran/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/LPnetlib/lpi_gran/micro_spy_454_371.png}} & \makecell{ LPnetlib/ \\ \quad lpi\_gran \\ $2658 \times 2525$ ($20111$)} \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Norris/heart3/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Norris/heart3/micro_spy_128_128.png}} & \makecell{ Norris/ \\ \quad heart3 \\ $2339 \times 2339$ ($682797$)} \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Rajat/rajat26/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/Rajat/rajat26/micro_spy_10186_10186.png}} & \makecell{ Rajat/ \\ \quad rajat26 \\ $51032 \times 51032$ ($249302$)} \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/TAMU_SmartGridCenter/ACTIVSg70K/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/TAMU_SmartGridCenter/ACTIVSg70K/micro_spy_62062_62062.png}} & \makecell{ TAMU\_SmartGridCenter/ \\ \quad ACTIVSg70K \\ $69999 \times 69999$ ($238627$)} \\
\raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/TSOPF/TSOPF_RS_b678_c1/spy.png}}\vspace{1pt} & \raisebox{-.5\height}{\includegraphics[width=1.7cm]{results/data/TSOPF/TSOPF_RS_b678_c1/micro_spy_942_248.png}} & \makecell{ TSOPF/ \\ \quad TSOPF\_RS\_b678\_c1 \\ $18696 \times 18696$ ($4396289$)} \\
\end{tabular}


==> VBR arxiv/results/median_1dvbr_critical.tex <==
$16.9$


==> VBR arxiv/results/median_1dvbr_speedup.tex <==
$2.22$$\times$


==> VBR arxiv/results/number_of_matrices.tex <==
20

==> VBR arxiv/results/results_spread.tex <==
\setlength{\tabcolsep}{2pt}\begin{tabular}{rp{12pt}rrrp{12pt}rrrp{12pt}rrr}
\multicolumn{1}{r}{\textbf{Partitioner}} &  & \multicolumn{3}{c}{\textbf{Memory Used}} &  & \multicolumn{3}{c}{\textbf{Multiply Time}} &  & \multicolumn{3}{c}{\textbf{Critical Point}}\\\cline{3-5}\cline{7-9}\cline{11-13}
\multicolumn{1}{r}{} &  & \multicolumn{1}{r}{\textbf{Q. 1}} & \multicolumn{1}{r}{\textbf{Med.}} & \multicolumn{1}{r}{\textbf{Q. 3}} &  & \multicolumn{1}{r}{\textbf{Q. 1}} & \multicolumn{1}{r}{\textbf{Med.}} & \multicolumn{1}{r}{\textbf{Q. 3}} &  & \multicolumn{1}{r}{\textbf{Q. 1}} & \multicolumn{1}{r}{\textbf{Med.}} & \multicolumn{1}{r}{\textbf{Q. 3}}\\
\hline
\textbf{Strict 1D-VBR} &   & $0.6$ & $0.808$ & $1$ &   & $0.573$ & $0.886$ & $1.17$ &   & $6.57$ & $46.1$ & $\infty$\\
\textbf{Overlap(0.9) 1D-VBR} &   & $0.615$ & $0.746$ & $0.918$ &   & $0.338$ & $0.545$ & $0.858$ &   & $10.9$ & $18.4$ & $68.3$\\
\textbf{Overlap(0.8) 1D-VBR} &   & $0.616$ & $0.746$ & $0.918$ &   & $0.338$ & $0.546$ & $0.902$ &   & $11.2$ & $18.4$ & $92.5$\\
\textbf{Overlap(0.7) 1D-VBR} &   & $0.619$ & $0.746$ & $0.918$ &   & $0.331$ & $0.547$ & $0.904$ &   & $10.9$ & $19$ & $69$\\
\textbf{Min Blocks 1D-VBR} &   & $0.606$ & $0.84$ & $1.32$ &   & $0.351$ & $0.493$ & $0.806$ &   & $13.9$ & $19$ & $66.3$\\
\textbf{Min Memory 1D-VBR} &   & $0.562$ & $0.633$ & $0.806$ &   & $0.347$ & $0.535$ & $0.723$ &   & $11.7$ & $17.3$ & $32.2$\\
\textbf{Min Compute 1D-VBR} &   & $0.585$ & $0.664$ & $0.857$ &   & $0.317$ & $0.45$ & $0.589$ &   & $12.4$ & $16.9$ & $29.1$\\
\textbf{Strict VBR} &   & $0.521$ & $0.696$ & $0.983$ &   & $0.543$ & $1.55$ & $2.16$ &   & $29.9$ & $\infty$ & $\infty$\\
\textbf{Overlap(0.9) VBR} &   & $0.575$ & $0.819$ & $1.18$ &   & $0.508$ & $0.769$ & $1.52$ &   & $28.8$ & $71.4$ & $\infty$\\
\textbf{Overlap(0.8) VBR} &   & $0.59$ & $0.834$ & $1.19$ &   & $0.487$ & $0.729$ & $1.56$ &   & $28.7$ & $68$ & $\infty$\\
\textbf{Overlap(0.7) VBR} &   & $0.605$ & $0.847$ & $1.2$ &   & $0.501$ & $0.777$ & $1.55$ &   & $28.5$ & $79.2$ & $\infty$\\
\textbf{Min Blocks VBR} &   & $0.67$ & $1.06$ & $2.8$ &   & $0.411$ & $0.573$ & $1.81$ &   & $29$ & $47.1$ & $\infty$\\
\textbf{Min Memory VBR} &   & $0.432$ & $0.56$ & $0.75$ &   & $0.451$ & $0.6$ & $1.31$ &   & $38.9$ & $62.1$ & $\infty$\\
\textbf{Min Compute VBR} &   & $0.556$ & $0.721$ & $1.06$ &   & $0.33$ & $0.512$ & $1.11$ &   & $36.2$ & $49.7$ & $\infty$\\
\end{tabular}


==> VBR arxiv/thebiggadgetmatrix.tex <==
$
\left[\begin{array}{cccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccccc}\cline{1-1} \cline{2-2} \cline{6-6} \cline{9-9} \cline{12-12} \cline{15-15} \cline{21-21} \cline{22-22} \cline{26-26} \cline{29-29} \cline{32-32} \cline{35-35} \cline{41-41} \cline{42-42} \cline{46-46} \cline{49-49} \cline{52-52} \cline{55-55} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{6-6} \cline{9-9} \cline{12-12} \cline{15-15} \cline{18-18} \cline{21-21} \cline{22-22} \cline{23-23} \cline{26-26} \cline{29-29} \cline{32-32} \cline{35-35} \cline{38-38} \cline{41-41} \cline{42-42} \cline{43-43} \cline{46-46} \cline{49-49} \cline{52-52} \cline{55-55} \cline{58-58} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} \cline{6-6} \cline{9-9} \cline{12-12} \cline{18-18} \cline{23-23} \cline{26-26} \cline{29-29} \cline{32-32} \cline{38-38} \cline{43-43} \cline{46-46} \cline{49-49} \cline{52-52} \cline{58-58} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{21-21} \cline{22-22} \cline{23-23} \cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{21-21} \cline{22-22} \cline{23-23} \cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{21-21} \cline{22-22} \cline{23-23} \cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{21-21} \cline{22-22} \cline{23-23} \cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{21-21} \cline{22-22} \cline{23-23} \cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{21-21} \cline{22-22} \cline{23-23} \cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{21-21} \cline{22-22} \cline{41-41} \cline{42-42} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{21-21} \cline{22-22} \cline{41-41} \cline{42-42} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} \cline{23-23} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} \cline{23-23} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} \cline{6-6} \cline{9-9} \cline{12-12} \cline{15-15} \cline{61-61} \cline{66-66} \cline{69-69} \cline{72-72} \cline{75-75} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{6-6} \cline{9-9} \cline{12-12} \cline{15-15} \cline{18-18} \cline{61-61} \cline{62-62} \cline{63-63} \cline{66-66} \cline{69-69} \cline{72-72} \cline{75-75} \cline{78-78} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{6-6} \cline{9-9} \cline{12-12} \cline{18-18} \cline{62-62} \cline{63-63} \cline{66-66} \cline{69-69} \cline{72-72} \cline{78-78} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{61-61} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{61-61} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{3-3} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{23-23} \cline{26-26} \cline{29-29} \cline{32-32} \cline{35-35} \cline{62-62} \cline{63-63} \cline{66-66} \cline{69-69} \cline{72-72} \cline{75-75} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{23-23} \cline{26-26} \cline{29-29} \cline{32-32} \cline{35-35} \cline{38-38} \cline{61-61} \cline{62-62} \cline{63-63} \cline{66-66} \cline{69-69} \cline{72-72} \cline{75-75} \cline{78-78} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{26-26} \cline{29-29} \cline{32-32} \cline{38-38} \cline{61-61} \cline{62-62} \cline{63-63} \cline{66-66} \cline{69-69} \cline{72-72} \cline{78-78} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{23-23} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{23-23} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{23-23} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{23-23} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{23-23} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{23-23} \cline{61-61} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{61-61} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{21-21} \cline{22-22} \cline{61-61} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{23-23} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{23-23} \cline{62-62} \cline{63-63} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{43-43} \cline{46-46} \cline{49-49} \cline{52-52} \cline{55-55} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} \cline{43-43} \cline{46-46} \cline{49-49} \cline{52-52} \cline{55-55} \cline{58-58} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} \cline{46-46} \cline{49-49} \cline{52-52} \cline{58-58} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} \cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{41-41} \cline{42-42} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{43-43} 
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\end{array}\right]
$


==> VBR arxiv/ubcsr_example.tex <==
\resizebox{0.5\width}{!}{$\left[\begin{array}{ccccccccc}\cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} \cline{9-9} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}\\\cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\end{array}\right]$}

\subcaption{The stored entries of $A$ in UBCSR format.}\label{fig:ubcsr-example}


==> VBR arxiv/vbl_example.tex <==
\resizebox{0.5\width}{!}{$\left[\begin{array}{ccccccccc}\cline{3-3} \cline{4-4} \cline{5-5} \cline{9-9} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} 
\multicolumn{1}{|c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{4-4} \cline{5-5} \cline{6-6} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\\cline{3-3} \cline{8-8} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\\cline{2-2} \cline{3-3} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{5-5} \cline{6-6} \cline{7-7} \cline{9-9} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{5-5} \cline{6-6} \cline{7-7} \cline{9-9} 
\end{array}\right]$}

\subcaption{The stored entries of $A$ in 1D-VBL format.}\label{fig:vbl-example}


==> VBR arxiv/vbr_example.tex <==
\resizebox{0.5\width}{!}{$\left[\begin{array}{ccccccccc}\cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{9-9} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{x}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{0}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{8-8} 
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\
\multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c}{}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c}{}\\\cline{1-1} \cline{2-2} \cline{3-3} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{8-8} \cline{9-9} 
\multicolumn{1}{|c}{0}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\
\multicolumn{1}{|c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c}{0}& \multicolumn{1}{c}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{x}& \multicolumn{1}{c|}{}& \multicolumn{1}{c|}{x}\\\cline{1-1} \cline{2-2} \cline{4-4} \cline{5-5} \cline{6-6} \cline{7-7} \cline{9-9} 
\end{array}\right]$}

\subcaption{The stored entries of $A$ in VBR format. Here, $\Pi = [1{:}1, 2{:}4, 5{:}6, 7{:}8]$ and $\Phi = [1{:}2, 3{:}3, 4{:}6, 7{:}7, 8{:}8, 9{:}9]$.}\label{fig:vbr-example}

